Large-Scale Clustering Based on Data Compression

This paper considers the clustering problem for large data sets. We propose an approach based on distributed optimization. The clustering problem is formulated as an optimization problem of maximizing the classification gain. We show that the optimization problem can be reformulated and decomposed into small-scale sub optimization problems by using the Dantzig-Wolfe decomposition method. Generally speaking, the Dantzig-Wolfe method can only be used for convex optimization problems, where the duality gaps are zero. Even though, the considered optimization problem in this paper is non-convex, we prove that the duality gap goes to zero, as the problem size goes to infinity. Therefore, the Dantzig-Wolfe method can be applied here. In the proposed approach, the clustering problem is iteratively solved by a group of computers coordinated by one center processor, where each computer solves one independent small-scale sub optimization problem during each iteration, and only a small amount of data communication is needed between the computers and center processor. Numerical results show that the proposed approach is effective and efficient.

==> thebib.tex <==
\begin{thebibliography}{99}

%\small

%\footnotesize


%\setlength{\parskip}{0pt}




\bibitem{azuma67} K. Azuma,
``Weighted sums of certain dependent random variables'', Tohoku
Mathematical Journal, vol. 19, no. 3, pp. 357-367, 1967.


\bibitem{chen77}W.H. Chen and C.H. Smith, ``Adaptive coding of monochrome and color
images'', {\it IEEE Transactions on Communications}, vol. 25, pp.
1285-1292, November 1977.


\bibitem{cover}T.M. cover, and J.A. Thomas,
{\it Elements of Information Theory},  John~Wiley, 1991.


\bibitem{dempster77} A. Dempster, N. Laird, and D. Rubin, ``Maximum likelihood from incomplete data via the EM
algorithm'', {\it Journal of the Royal Statistical Society, Series
B}, vol. 39, no. 1, pp. 1-38, 1977.


\bibitem{duda00} R. Duda, P. Hart and D. Stork,
{\it Pattern Classification} (2nd Edition), John Wiley \& Sons 2000.



\bibitem{janson98}S. Janson,
``On concentration of probability'',   {\it Proceedings of Workshop
on Probabilistic Combinatorics at the Paul Erdos Summer Research
Center, Budapest 1998},  pp. 289-301.



\bibitem{joshi97} R.L. Joshi, H. Jafarkhani, J.H. Kasner, T.R.
Fischer, N. Farvardin, M.W. Marcellin, and R.H. Bamberger,
``Comparison of different methods of classification in subband
coding of images'', {\it IEEE Transactions on Image Processing},
vol. 6, no. 11, pp. 1473 - 1486, November 1997.




\bibitem{ma08} X. Ma, ``Information theoretic analysis of the data compression based signal classification
algorithm'', working paper.


\bibitem{sezgin04}M. Sezgin and B. Sankur, ``Survey over image thresholding
techniques and quantitative performance evaluation'', {\it Journal
of Electronic Imaging}, vol. 13, no. 1, pp. 146-165, 2004.


\bibitem{srinvasan05}U. Srinivasan, S. Pfeiffer, S. Nepal, M. Lee, L. Gu, and S.
Barrass, ``A Survey of MPEG-1 Audio, Video and Semantic Analysis
 Techniques'',
{\it Journal Multimedia Tools and Applications}, vol. 27, no. 1, pp.
105-141,  August 2005.



\bibitem{theodoridis06}S. Theodoridis, and K. Koutroumbas, {\it Pattern
Recognition}, Third Edition, Academic Press,  2006.



\bibitem{tse92}Y.-T. Tse, ``Video coding using global/local motion compensation, classified subband coding
, uniform threshold quantization and arithmetic coding'', Ph.D.
thesis, University of California, Los Angeles, 1992.


\bibitem{wachter06}
A. Wachter and L. T. Biegler, ``On the implementation of a
primal-dual interior point filter line search algorithm for
large-scale nonlinear programming'', {\it Mathematical Programming},
vol. 106, no. 1, pp. 25-57, 2006. The software package is available
from https://projects.coin-or.org/Ipopt.


\bibitem{woods86}J.W. Woods and S.D. O'Neil, ``Subband coding of
images'', {\it IEEE Transactions on Acoustics, Speech, and Signal
Processing,} vol. 34, pp. 1278-1288, October 1986.


\bibitem{yoo99} Y. Yoo, A. Ortega, and B. Yu,
``Image subband coding using context-based classification and
adaptive quantization'',  {\it IEEE Transactions on Image
Processing,} vol. 8, pp. 1702-1715, 1999.


















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




















\end{thebibliography}


































%

